Graph-GRPO: Dependency-Aware Credit Assignment for Generative E-commerce Search Relevance

Search relevance modeling is a core task in e-commerce search systems, assessing how well a user query matches candidate products. Rather than relying on a single holistic matching signal, relevance judgment often requires structured reasoning over query understanding, product understanding, and facet-level matching. With large language models (LLMs), this process is increasingly formulated as chain-of-thought (CoT) reasoning and optimized with reinforcement learning (RL). However, existing RL methods mainly rely on outcome-level rewards and treat the entire reasoning chain as a single optimization unit. This makes it difficult to distinguish faulty reasoning steps from correct intermediate ones, leading to misaligned credit assignment. Although process-reward methods provide denser supervision, they often treat reasoning steps independently and ignore dependency-driven error propagation, making responsibility attribution difficult and limiting the optimization of structured relevance reasoning. We propose Graph-GRPO, a graph-structured extension of GRPO for multi-component relevance reasoning. Graph-GRPO constructs a relevance reasoning dependency graph, where CoT steps are modeled as nodes and their logical dependencies as edges. It propagates outcome-level rewards over the graph to derive step-level credit signals, enabling more accurate fine-grained credit assignment. We further introduce a main-loss-driven controller that adaptively adjusts edge-wise credit-propagation coefficients. Together with CoT random masking for supervised policy initialization and graph-node-based multi-head distillation, we build a trainable and deployable framework for generative relevance modeling. Extensive offline evaluations and online A/B tests on a leading e-commerce platform demonstrate that the Graph-GRPO-based framework improves relevance classification metrics and key engagement metrics.

==> chapter/deprecated/abstract_v0.tex <==
Search relevance modeling is a core task in e-commerce search systems, aiming to assess the matching degree between a user query and a candidate product. This task requires understanding the entity and adjective information in both the query and the product. 
In recent years, large language models have been introduced into search relevance modeling due to their strong semantic understanding and reasoning capabilities. 
This has shifted the task from single-step label prediction to structured chain-of-thought reasoning. 
To further optimize the reasoning process, reinforcement learning methods have been increasingly applied. 
However, existing reinforcement learning methods mainly rely on sparse outcome-level rewards, making it difficult to provide fine-grained supervision for the reasoning process. 
Although process rewards constructed from manual rules or external reward models can provide denser supervision, they are costly to construct and often unstable in practice. 
Moreover, existing methods often overlook the logical dependencies among reasoning components, which weakens the optimization of the reasoning process.

To address fine-grained credit assignment in relevance reasoning, we propose Graph-GRPO, a reinforcement learning method based on graph-structured credit assignment. Graph-GRPO constructs a relevance reasoning dependency graph to propagate outcome-level rewards into structured node-level feedback, enabling more precise responsibility attribution across reasoning components. We further introduce a main-loss-driven learnable graph coefficient mechanism to adaptively adjust credit propagation during policy optimization. Together with CoT random masking for supervised policy initialization and graph-node-based multi-head distillation, we build a trainable and deployable framework for generative relevance modeling. Extensive offline evaluations and online A/B tests demonstrate that the proposed framework significantly improves key relevance and business metrics and further enhances the user experience of e-commerce search systems.

==> chapter/deprecated/abstract_v1.tex <==
Search relevance modeling is a core task in e-commerce search systems, aiming to assess the matching degree between a query and candidate products. This task requires deep reasoning in understanding both query and product semantics, as well as capturing complex matching patterns in e-commerce scenarios. In recent years, large language models have been introduced into e-commerce search relevance due to their strong semantic understanding and reasoning capabilities. This has shifted the task from single-step label prediction to structured chain-of-thought reasoning. To further optimize the reasoning process, reinforcement learning methods have been increasingly adopted in industrial e-commerce search. Existing methods improve the effectiveness of reinforcement by introducing denser reward signals to alleviate sparse feedback. However, they overlook the logical dependencies among the reasoning components in search relevance.

To address fine-grained credit assignment in relevance reasoning, we propose Graph-GRPO, a reinforcement learning method based on graph-structured credit assignment. Graph-GRPO constructs a relevance reasoning dependency graph to propagate outcome-level rewards into structured node-level feedback, enabling more precise responsibility attribution across reasoning components. We further introduce a main-loss-driven mechanism to adaptively adjust the credit propagation ratio. Combining CoT with random masking and multi-head distillation, we build a trainable and deployable framework for generative relevance modeling. Extensive offline evaluations and online A/B tests demonstrate that the proposed framework significantly improves the user experience of e-commerce search systems.
